Research Vision: Multi-Agent Path Planning for Cops And Robbers Via Reactive Synthesis

We propose the problem of multi-agent path planning for a generalization of the classic Cops and Robbers game via reactive synthesis. Specifically, through the application of LTLt and Coordination Synthesis, we aim to check whether various Cops and Robbers games are realizable (a strategy exists for the cops which guarantees they catch the robbers). Additionally, we construct this strategy as an executable program for the multiple system players in our games. In this paper we formalize the problem space, and propose potential directions for solutions. We also show how our formalization of this generalized cops and robbers game can be mapped to a broad range of other problems in the reactive program synthesis space.

==> code.tex <==
\begin{small}
\begin{verbatim}
# Returns the checkerboard color based on parity.
def checker(x, y):
    if (x + y) % 2 == 0:
         return "white"
    else:
         return "black"

# Given a starting point, L_plot paints a specific sequence of cells black.
# At each step it checks if the computed cell is still in the L region.
# If a point falls outside, the function returns immediately without further painting.
def L_plot(starting_point):
    x, y = starting_point
    set_color_to_black((x, y))    # Paint starting point black

    # First vertical segment: two steps
    for i in range(1, 3):
         if phi(x, y + i) != "L-shape":
              return (x, y + i)
         set_color_to_black((x, y + i))
         # Update current position to the new point
         x, y = x, y + i

    # Horizontal move: one step to the right
    if phi(x + 1, y) != "L-shape":
         return (x + 1, y)
    set_color_to_black((x + 1, y))
    x, y = x + 1, y

    # Second vertical segment: two steps to the right (or using x-offset)
    for i in range(1, 3):
         if phi(x + i, y) != "L-shape":
              return (x + i, y)
         set_color_to_black((x + i, y))
         x, y = x + i, y

    # Final horizontal move: one step upward
    if phi(x, y + 1) != "L-shape":
         return (x, y + 1)
    set_color_to_black((x, y + 1))
    x, y = x, y + 1

    return (x, y)


# Generates the L pattern starting from an initial point.
# (Here, the starting coordinates are chosen so that (x+y) mod 100 == 25.)
def Generate_L_Plot():
    starting_point = (round(25/2), int(25/2))
    # NUM_ITERATIONS defines how many iterations we simulate.
    for _ in range(NUM_ITERATIONS):
         if not in_L_region(starting_point):
              break
         starting_point = L_plot(starting_point)
    return

# phi returns "L-shape" if the cell (x,y) is in an L tile,
# otherwise it returns the checkerboard color (or "background").
def phi(x, y):
    if (x + y) % 100 < 25 or (x + y) % 100 >= 75:
         return checker(x, y)
    elif (x, y) in L_tile_black_cells:
         return "L-shape"
    else:
         return "background"

# This is the final function that determines whether a given cell is white or black.
# It assumes that Generate_L_Plot has been run over a sufficiently large region.
def cell_color(x, y):
    # Cells in the checkerboard region
    if (x + y) % 100 < 25 or (x + y) % 100 >= 75:
         return checker(x, y)
    else:
         # In the L region, cells that have been painted by the L_plot routine
         # are black; others default to the checkerboard color.
         if (x, y) in L_tile_black_cells:
              return "black"
         else:
              return checker(x, y)
\end{verbatim}
\end{small}
